Compositionality with Primitives: A Unified View from Euclidean to Hyperbolic Vision-Language Models

Compositional zero-shot learning (CZSL) aims to recognize novel combinations of previously observed objects and attributes. Prior work showed that large-scale vision-language models encode decomposable semantic structures that can be recomposed to enable generalization. The Geodesically Decomposable Embeddings (GDE) framework formalizes this by identifying directions in the tangent space at the Frechet mean of the embedding distribution, which encode primitive visual concepts. Unseen attribute-object compositions can be synthesized through vector addition of these primitives. We revisit the assumption that compositional generalization requires explicit attribute-object pair re-composition. By means of new compositional scoring functions and extensive evaluations, we show that directly using the decomposed primitives suffices for recognizing unseen compositions. In that, we gain insights on how the geometry of the embedding manifold (Euclidean, spherical, or hyperbolic) and dataset structure affect compositional reasoning. Across models (CLIP, DINOv2, MERU, HyCoCLIP), we show that compositional structure consistently emerges as primitive representations, enabling inference on CZSL benchmarks (MIT-States, VAW-CZSL, UT-Zappos50K, Clothing16K) and group robustness on Waterbirds and CelebA. Code: https://github.com/nis-research/Compositionality-with-Primitives.

==> figures/geometries/euclidean.tex <==
\begin{tikzpicture}
% ---------- inline shape macros for subscripts ----------
\newcommand{\redsquare}{\tikz[baseline=-0.5ex]\fill[red!70] (0,0) rectangle (1.6ex,1.6ex);}
\newcommand{\redtriangle}{\tikz[baseline=-0.5ex]\fill[red!70] (0,0) -- (1.6ex,0) -- (0.8ex,1.4ex) -- cycle;}
\newcommand{\bluesquare}{\tikz[baseline=-0.5ex]\fill[blue!70] (0,0) rectangle (1.6ex,1.6ex);}
\newcommand{\bluetriangle}{\tikz[baseline=-0.5ex]\fill[blue!70] (0,0) -- (1.6ex,0) -- (0.8ex,1.4ex) -- cycle;}

% ---------- pseudo-3D euclidean space (parallelogram floor) ----------
\fill[gray!15, opacity=0.6]
    (-2.8,-2.2) -- (3.2,-2.2) -- (2.2,2.6) -- (-3.8,2.6) -- cycle;
\draw[thick, gray!60]
    (-2.8,-2.2) -- (3.2,-2.2) -- (2.2,2.6) -- (-3.8,2.6) -- cycle;

% ---------- faint grid lines for 3D perspective feel ----------
\foreach \t in {0.2,0.4,0.6,0.8}{
    \draw[gray!30, very thin]
        ($(-2.8,-2.2)!\t!(-3.8,2.6)$) -- ($(3.2,-2.2)!\t!(2.2,2.6)$);
}
\foreach \t in {0.2,0.4,0.6,0.8}{
    \draw[gray!30, very thin]
        ($(-2.8,-2.2)!\t!(3.2,-2.2)$) -- ($(-3.8,2.6)!\t!(2.2,2.6)$);
}

% ---------- key points (suspended in the pseudo-3D space) ----------
\coordinate (A) at (-1.8,1.2);   % red square cluster
\coordinate (B) at (0,0);        % mu center
\coordinate (C) at (1.8,1.2);    % red triangle cluster
\coordinate (D) at (-1.8,-1.2);  % blue square cluster
\coordinate (E) at (1.2,-0.2);   % blue triangle cluster

% ---------- top-left red square cluster ----------
\fill[red!60] (A) rectangle ++(0.18,0.18);
\foreach \x/\y in {-2.2/1.8, -2.0/1.6, -1.6/1.9, -1.9/1.3, -2.3/1.4}{
    \fill[red!30] (\x,\y) rectangle ++(0.12,0.12);
}
% ---------- top-right red triangle cluster ----------
\fill[red!70] (C) -- ++(0.15,0) -- ++(-0.075,0.13) -- cycle;
\foreach \x/\y in {2.1/1.6, 1.9/1.8, 2.3/1.7, 1.8/1.3}{
    \fill[red!30] (\x,\y) -- ++(0.1,0) -- ++(-0.05,0.08) -- cycle;
}
% ---------- bottom-left blue square cluster ----------
\fill[blue!70] (D) rectangle ++(0.18,0.18);
\foreach \x/\y in {-2.2/-1.6, -2.0/-1.8, -1.7/-1.7, -2.3/-1.3}{
    \fill[blue!30] (\x,\y) rectangle ++(0.12,0.12);
}
% ---------- bottom-right blue triangle cluster ----------
\fill[blue!70] (E) -- ++(0.15,0) -- ++(-0.075,0.13) -- cycle;
\foreach \x/\y in {1.6/-0.8, 1.9/-0.9, 1.7/-1.1, 1.4/-0.7}{
    \fill[blue!30] (\x,\y) -- ++(0.1,0) -- ++(-0.05,0.08) -- cycle;
}

% ---------- central point mu ----------
\fill (B) circle (2pt);
\node at (0.1,-0.25) {$\mu$};

% ---------- straight vectors from mu to each cluster (euclidean: no rotation) ----------
\draw[->, black] (B) -- (A)
    node[midway, above, sloped, font=\small] {$\mathbf{v}_{\redsquare}$};
\draw[->, black] (B) -- (C)
    node[midway, above, sloped, font=\small] {$\mathbf{v}_{\redtriangle}$};
\draw[->, black] (B) -- (D)
    node[midway, below, sloped, font=\small] {$\mathbf{v}_{\bluesquare}$};
\draw[->, black] (B) -- (E)
    node[midway, below, sloped, font=\small] {$\mathbf{v}_{\bluetriangle}$};
\end{tikzpicture}

==> figures/geometries/hyperboloid.tex <==
\begin{tikzpicture}
% ---------- inline shape macros for subscripts ----------
\newcommand{\redsquare}{\tikz[baseline=-0.5ex]\fill[red!70] (0,0) rectangle (1.6ex,1.6ex);}
\newcommand{\redtriangle}{\tikz[baseline=-0.5ex]\fill[red!70] (0,0) -- (1.6ex,0) -- (0.8ex,1.4ex) -- cycle;}
\newcommand{\bluesquare}{\tikz[baseline=-0.5ex]\fill[blue!70] (0,0) rectangle (1.6ex,1.6ex);}
\newcommand{\bluetriangle}{\tikz[baseline=-0.5ex]\fill[blue!70] (0,0) -- (1.6ex,0) -- (0.8ex,1.4ex) -- cycle;}

% ============================================================
% Top-down view of hyperbolic space (Poincaré-disk-like)
% Tree-like composition flowing left -> right:
%   μ (root, left)  --->  gray square + gray triangle (intermediate)
%                  --->  red/blue square + red/blue triangle clusters (leaves, right)
% ============================================================

% ---------- ambient disk (the hyperbolic "page" seen top-down) ----------
\fill[blue!15, opacity=0.6] (0,0) circle (3.6);
\draw[thick, blue!40!black, opacity=0.6] (0,0) circle (3.6);

% ============================================================
% Tangent plane — sits around the gray intermediate nodes (middle)
% Trapezoid with the LEFT edge shorter than the RIGHT edge,
% denoting the curvature of hyperbolic space (things stretch outward).
% ============================================================
\coordinate (TPbl) at (-2.6,-2.6);   % bottom-left  (short side)
\coordinate (TPtl) at (-2.6, 2.6);   % top-left     (short side)
\coordinate (TPtr) at ( 2.6, 2.6);   % top-right    (long side)
\coordinate (TPbr) at ( 2.4,-2.6);   % bottom-right (long side)
\fill[orange!15, opacity=0.55] (TPbl) -- (TPtl) -- (TPtr) -- (TPbr) -- cycle;
% \draw[orange!60!black, thick, opacity=0.75] (TPbl) -- (TPtl) -- (TPtr) -- (TPbr) -- cycle;

% ============================================================
% Key points (tree structure)
% ============================================================
\coordinate (MU) at (0.2, -0.2);     % root μ (far left)
\coordinate (GS) at ( 1.2, 0.2);     % gray square (intermediate, upper)
\coordinate (GT) at ( -1.2, 0.3);     % gray triangle (intermediate, lower)

% Leaf cluster centers (further right, branching out)
\coordinate (A) at ( 2.4, 1.4);      % red square cluster
\coordinate (D) at ( 2.4, -1.2);      % blue square cluster (branches from gray square)
\coordinate (C) at ( -2.4, 1.2);      % red triangle cluster (branches from gray triangle)
\coordinate (E) at ( -2.4, -1.4);      % blue triangle cluster

% ============================================================
% Tree edges (curved slightly to suggest hyperbolic geodesics in top-down view)
% ============================================================
% μ -> gray nodes
\draw[dashed, thick, gray!70] (MU) to[out=20,in=180]  (GS);
\draw[dashed, thick, gray!70] (MU) to[out=-20,in=180] (GT);
% gray square -> red square, blue square
\draw[dashed, thick, gray!70] (GS) to[out=20,in=190]  (A);
\draw[dashed, thick, gray!70] (GS) to[out=-20,in=170] (D);
% gray triangle -> red triangle, blue triangle
\draw[dashed, thick, gray!70] (GT) to[out=20,in=190]  (C);
\draw[dashed, thick, gray!70] (GT) to[out=-20,in=170] (E);

% ============================================================
% Intermediate gray nodes (uncoloured square + triangle)
% ============================================================
\fill[gray!60] ($(GS)+(-0.09,-0.09)$) rectangle ++(0.18,0.18);
\fill[gray!60] (GT) ++(-0.09,-0.08) -- ++(0.18,0) -- ++(-0.09,0.16) -- cycle;

% ============================================================
% Leaf clusters (further right)
% ============================================================
% Red square cluster (top-right)
\fill[red!60] (A) rectangle ++(0.18,0.18);
\foreach \dx/\dy in {-0.35/0.35, -0.15/0.2, 0.2/0.3, 0.3/-0.1, -0.3/-0.15}{
    \fill[red!30] ($(A)+(\dx,\dy)$) rectangle ++(0.12,0.12);
}
% Blue square cluster (upper-middle-right)
\fill[blue!70] (D) rectangle ++(0.18,0.18);
\foreach \dx/\dy in {-0.35/0.25, -0.15/0.3, 0.2/0.1, 0.3/-0.15, -0.3/-0.2}{
    \fill[blue!30] ($(D)+(\dx,\dy)$) rectangle ++(0.12,0.12);
}
% Red triangle cluster (lower-middle-right)
\fill[red!70] (C) -- ++(0.15,0) -- ++(-0.075,0.13) -- cycle;
\foreach \dx/\dy in {-0.35/-0.2, -0.1/-0.25, 0.25/-0.1, 0.2/0.15, -0.3/0.1}{
    \fill[red!30] ($(C)+(\dx,\dy)$) -- ++(0.1,0) -- ++(-0.05,0.08) -- cycle;
}
% Blue triangle cluster (bottom-right)
\fill[blue!70] (E) -- ++(0.15,0) -- ++(-0.075,0.13) -- cycle;
\foreach \dx/\dy in {-0.35/-0.2, -0.1/-0.15, 0.25/0.05, 0.2/0.2, -0.3/0.25}{
    \fill[blue!30] ($(E)+(\dx,\dy)$) -- ++(0.1,0) -- ++(-0.05,0.08) -- cycle;
}

% ============================================================
% μ (root, on the left, before the gray nodes)
% ============================================================
\fill (MU) circle (2pt);
\node[left=3pt] at (MU) {$\mu$};

% ============================================================
% Tangent vectors from μ toward each leaf cluster
% (straight arrows in the tangent plane; the dashed curves show the manifold geodesics)
% ============================================================
\draw[->, black] (MU) -- (A)
    node[midway, above, sloped, font=\small] {$\mathbf{v}_{\redsquare}$};
\draw[->, black] (MU) -- (D)
    node[midway, above, sloped, font=\small] {$\mathbf{v}_{\bluesquare}$};
\draw[->, black] (MU) -- (C)
    node[midway, below, sloped, font=\small] {$\mathbf{v}_{\redtriangle}$};
\draw[->, black] (MU) -- (E)
    node[midway, below, sloped, font=\small] {$\mathbf{v}_{\bluetriangle}$};
\end{tikzpicture}

==> figures/geometries/spherical.tex <==
\begin{tikzpicture}
% ---------- base circle (bottom half emphasis) ----------
\fill[blue!35, opacity=0.7] (0,0) circle (3);
% ---------- key points ----------
\coordinate (A) at (-1.8,1.2);   % red square (left top cluster center)
\coordinate (B) at (0,0);      % mu center
\coordinate (C) at (1.8,1.2);    % red triangle (right top)
\coordinate (D) at (-1.8,-1.2);  % blue square (bottom left)
\coordinate (E) at (1.2,-0.2);   % blue triangle (bottom right-ish)
% ---------- dashed trajectories ----------
\draw[dashed, thick, gray!70]
    (A) to[out=10,in=170] (B) to[out=10,in=160] (C);
\draw[dashed, thick, gray!70]
    (D) to[out=30,in=220] (B) to[out=-20,in=140] (E);

% ---------- top-left red square cluster ----------
\fill[red!60] (A) rectangle ++(0.18,0.18);
\foreach \x/\y in {-2.2/1.8, -2.0/1.6, -1.6/1.9, -1.9/1.3, -2.3/1.4}{
    \fill[red!30] (\x,\y) rectangle ++(0.12,0.12);
}
% ---------- top-right red triangle cluster ----------
\fill[red!70] (C) -- ++(0.15,0) -- ++(-0.075,0.13) -- cycle;
\foreach \x/\y in {2.1/1.6, 1.9/1.8, 2.3/1.7, 1.8/1.3}{
    \fill[red!30] (\x,\y) -- ++(0.1,0) -- ++(-0.05,0.08) -- cycle;
}
% ---------- bottom-left blue square cluster ----------
\fill[blue!70] (D) rectangle ++(0.18,0.18);
\foreach \x/\y in {-2.2/-1.6, -2.0/-1.8, -1.7/-1.7, -2.3/-1.3}{
    \fill[blue!30] (\x,\y) rectangle ++(0.12,0.12);
}
% ---------- bottom-right blue triangle cluster ----------
\fill[blue!70] (E) -- ++(0.15,0) -- ++(-0.075,0.13) -- cycle;
\foreach \x/\y in {1.6/-0.8, 1.9/-0.9, 1.7/-1.1, 1.4/-0.7}{
    \fill[blue!30] (\x,\y) -- ++(0.1,0) -- ++(-0.05,0.08) -- cycle;
}
% ---------- background slanted band ----------
\fill[orange!10, thick, opacity=0.35, rotate around={-8:(0,1)}]
    (-4,-2.5) rectangle (4,2.5);

% ---------- inline shape macros for subscripts ----------
\newcommand{\redsquare}{\tikz[baseline=-0.5ex]\fill[red!70] (0,0) rectangle (1.6ex,1.6ex);}
\newcommand{\redtriangle}{\tikz[baseline=-0.5ex]\fill[red!70] (0,0) -- (1.6ex,0) -- (0.8ex,1.4ex) -- cycle;}
\newcommand{\bluesquare}{\tikz[baseline=-0.5ex]\fill[blue!70] (0,0) rectangle (1.6ex,1.6ex);}
\newcommand{\bluetriangle}{\tikz[baseline=-0.5ex]\fill[blue!70] (0,0) -- (1.6ex,0) -- (0.8ex,1.4ex) -- cycle;}

% ---------- central point mu ----------
\fill (B) circle (2pt);
\node at (0.1,-0.25) {$\mu$};

% ---------- vectors from mu to each cluster (aligned to orange band perspective) ----------
\begin{scope}[rotate around={-8:(0,1)}]
    \draw[->, black] (B) -- (A)
        node[midway, above, sloped, font=\small] {$\mathbf{v}_{\redsquare}$};
    \draw[->, black] (B) -- (C)
        node[midway, above, sloped, font=\small] {$\mathbf{v}_{\redtriangle}$};
    \draw[->, black] (B) -- (D)
        node[midway, below, sloped, font=\small] {$\mathbf{v}_{\bluesquare}$};
    \draw[->, black] (B) -- (E)
        node[midway, below, sloped, font=\small] {$\mathbf{v}_{\bluetriangle}$};
\end{scope}

% ---------- outline circle ----------
\draw[thick] (0,0) circle (3);
\end{tikzpicture}


==> figures/paradigm.tex <==
% Cleaner evaluation paradigms figure
% Requires: tikz, tikzlibrary{arrows.meta, positioning, calc, backgrounds}

\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
  font=\sffamily\small,
  >=Stealth,
  attvec/.style   = {->, line width=2.1pt, blue!65!cyan, cap=round},
  objvec/.style   = {->, line width=2.1pt, violet!80!magenta, cap=round},
  compvec/.style  = {->, line width=1.9pt, orange!90!red,
                     dash pattern=on 5pt off 2.5pt, cap=round},
  ghostatt/.style = {->, line width=1.1pt, blue!35!cyan!65, cap=round},
  ghostobj/.style = {->, line width=1.1pt, violet!45!magenta!65, cap=round},
  matcharrow/.style = {->, line width=1.4pt, red!70!orange, cap=round},
  cosdash/.style  = {dashed, line width=1.1pt, teal!70!cyan},
  panelbg/.style  = {fill=gray!6, rounded corners=5pt},
]

% ------------------------------------------------------------------
% Layout
% ------------------------------------------------------------------
\def\Lx{1.8}
\def\Rx{11.3}
\def\panelW{7.8}
\def\panelH{7.4}

\begin{scope}[on background layer]
  \fill[panelbg] (\Lx-1.0,-1.05) rectangle (\Lx+\panelW,\panelH);
  \fill[panelbg] (\Rx-1.0,-1.05) rectangle (\Rx+\panelW,\panelH);
\end{scope}

% ==================================================================
% LEFT PANEL
% ==================================================================
\def\lx{\Lx+1.0}

\filldraw[black] (\lx,0) circle (2.7pt)
  node[below left=1pt] {$\mu$};

\node[font=\sffamily\itshape\footnotesize, text=gray!70]
  at (\lx+2.9,-0.72) {Tangent space at $\mu$};

% attribute
\draw[attvec] (\lx,0) -- (\lx-0.75,3.35)
  node[pos=.68, left=4pt, text=blue!65!cyan] {$\mathbf{v}_a$};

% object
\draw[objvec] (\lx,0) -- (\lx+3.75,1.95)
  node[pos=.63, below=3pt, text=violet!80!magenta] {$\mathbf{v}_o$};

% composed prototype
\coordinate (pairtip) at (\lx+2.95,4.75);
\draw[compvec] (\lx,0) -- (pairtip);
\draw[gray!30, thin] (\lx-0.75,3.35) -- (pairtip);
\draw[gray!30, thin] (\lx+3.75,1.95) -- (pairtip);

\filldraw[orange!90!red] (pairtip) circle (3.4pt);
\node[anchor=west, text=orange!85!black] at ($(pairtip)+(0.16,0.05)$)
  {$\mathbf{v}_a+\mathbf{v}_o$};

% test image
\node[font=\Large] (tx) at (\lx+4.2,5.95) {$\bigstar$};
\node[above right=0pt and 1pt of tx] {$\mathbf{t}_x$};

\draw[matcharrow] (tx) -- ($(pairtip)+(0.02,0.10)$);
\node[font=\sffamily\itshape\footnotesize, text=red!70!orange]
  at (\lx+3.85,5.15) {match};

% alternative prototypes
\filldraw[gray!42] (\lx+0.2,4.35) rectangle ++(0.16,0.16);
\filldraw[gray!42] (\lx+5.15,3.45) rectangle ++(0.16,0.16);

\node[gray!55, font=\sffamily\footnotesize, anchor=east]
  at (\lx+0.12,4.43) {$\mathbf{v}_{a'}+\mathbf{v}_{o'}$};

\node[gray!55, font=\sffamily\footnotesize, anchor=west]
  at (\lx+5.38,3.53) {$\mathbf{v}_{a''}+\mathbf{v}_{o''}$};

% title
\node[font=\sffamily\bfseries] at (\Lx+3.0,\panelH-0.35)
  {(a) Pair-based};

% ==================================================================
% RIGHT PANEL
% ==================================================================
\def\Px{\Rx+1.6}
\filldraw[black] (\Px,0) circle (2.7pt)
  node[below left=1pt] {$\mu$};

\node[font=\sffamily\itshape\footnotesize, text=gray!70]
  at (\Px+2.9,-0.72) {Tangent space at $\mu$};

% winning attribute
\draw[attvec] (\Px,0) -- (\Px+0.8,4.2)
  node[pos=.78, right=3pt, text=blue!65!cyan] {$\mathbf{v}_{a_2}$};

% ghost attributes
\draw[ghostatt] (\Px,0) -- (\Px-1.15,3.35);
\draw[ghostatt] (\Px,0) -- (\Px-2.05,2.05);

\node[font=\sffamily\footnotesize, text=blue!35!cyan!70]
  at (\Px-1.55,3.55) {$\mathbf{v}_{a_1}$};

\node[font=\sffamily\footnotesize, text=blue!35!cyan!70]
  at (\Px-2.35,2.25) {$\mathbf{v}_{a_3}$};

% winning object
\draw[objvec] (\Px,0) -- (\Px+4.35,1.8)
  node[pos=.8, below right=2pt, text=violet!80!magenta] {$\mathbf{v}_{o_1}$};

% ghost objects
\draw[ghostobj] (\Px,0) -- (\Px+3.55,2.95);
\draw[ghostobj] (\Px,0) -- (\Px+4.95,0.55);

\node[font=\sffamily\footnotesize, text=violet!50!magenta!70]
  at (\Px+3.85,3.15) {$\mathbf{v}_{o_2}$};

\node[font=\sffamily\footnotesize, text=violet!50!magenta!70]
  at (\Px+5.2,0.55) {$\mathbf{v}_{o_3}$};

% test image
\node[font=\Large] (rtx) at (\Px+3.15,5.75) {$\bigstar$};
\node[above right=0pt and 1pt of rtx] {$\mathbf{t}_x$};

% cosine matches
\coordinate (attTip) at (\Px+0.72,5.55);
\coordinate (objTip) at (\Px+5.95,2.75);

\filldraw[teal!60!cyan] (attTip) circle (2.5pt);
\filldraw[teal!60!cyan] (objTip) circle (2.5pt);

\draw[cosdash] (rtx) -- (attTip);
\draw[cosdash] (rtx) -- (objTip);

\node[font=\sffamily\footnotesize, text=teal!70!cyan]
  at (\Px+0.9,5.8) {$\cos(\mathbf{v}_{a_2},\mathbf{t}_x)$};

\node[font=\sffamily\footnotesize, text=teal!70!cyan]
  at (\Px+5.5,2.5) {$\cos(\mathbf{v}_{o_1},\mathbf{t}_x)$};

% title
\node[font=\sffamily\bfseries] at (\Px+1.75,\panelH-0.35)
  {(b) Primitive-based};

% ==================================================================
% Legend
% ==================================================================
\def\Ly{-1.65}
\def\lx{\Lx+1.0}

\draw[attvec] (\lx,\Ly) -- ++(0.9,0);
\node[right=2pt, font=\sffamily\footnotesize] at (\lx+0.9,\Ly)
  {attribute};

\draw[objvec] (\lx+3.6,\Ly) -- ++(0.9,0);
\node[right=2pt, font=\sffamily\footnotesize] at (\lx+4.5,\Ly)
  {object};

\draw[compvec] (\lx+6.8,\Ly) -- ++(0.9,0);
\node[right=2pt, font=\sffamily\footnotesize] at (\lx+7.7,\Ly)
  {pair prototype};

\node[font=\normalsize] at (\lx+11.0,\Ly) {$\bigstar$};
\node[right=2pt, font=\sffamily\footnotesize] at (\lx+11.25,\Ly)
  {test image};

\end{tikzpicture}
}
\caption{%
  \textbf{Classification paradigms in tangent space.}
  %
  \emph{(a) Pair-based} (prior work): a prototype $\mathbf{v}_a + \mathbf{v}_o$ is
  constructed by adding the attribute and object directions, and the nearest prototype
  to the test embedding $\mathbf{t}_x$ is selected ($\hat{y} = \arg\min_{(a,o)}
  d(\mathbf{t}_x, \mathbf{v}_a + \mathbf{v}_o)$).
  The faded squares are the remaining pair prototypes in the open-world candidate set;
  classification requires computing the distance to every $(a,o)$ combination.
  This approach relies on the additivity hypothesis and degrades when attribute-object
  entanglement pushes the true pair centroid away from the additive sum.
  %
  \emph{(b) Primitive-based} (proposed): the attribute and object are scored
  independently via cosine similarity to each primitive direction
  ($\hat{a} = \arg\max_a \cos(\mathbf{v}_a, \mathbf{t}_x)$,\;
   $\hat{o} = \arg\max_o \cos(\mathbf{v}_o, \mathbf{t}_x)$),
  making no assumption about how the two directions combine.
  Faded arrows show the unchosen primitive directions; the teal dashed lines indicate
  the cosine similarity to the winning attribute and object.
  The additivity residual $r(a,o) = \|\mathbf{c}_{a,o} - (\mathbf{v}_a +
  \mathbf{v}_o)\|$ quantifies per-pair entanglement and predicts which paradigm
  succeeds.%
}
\label{fig:paradigms}
\end{figure}


==> figures/tangent/all.tex <==
% ==================================================================
% ROW 1: MANIFOLD MEANS
% ==================================================================
% Subfigure (a): Euclidean Means
\begin{minipage}[t]{0.33\linewidth}
    \centering
    \begin{tikzpicture}
        \node[anchor=south west, inner sep=0] (image) at (0,0) {
            % \vspace{-2ex}
            \includegraphics[width=\linewidth]{figures/tangent/sph_manifold_means.pdf}
        % \node[anchor=north west, fill=white, fill opacity=0.7, text opacity=1, inner sep=2pt] at (image.north west) {\textbf{(a)}};
        };
    \end{tikzpicture}
\end{minipage}%
% Subfigure (b): Spherical Means
\begin{minipage}[t]{0.33\linewidth}
    \centering
    \begin{tikzpicture}
        \node[anchor=south west, inner sep=0] (image) at (0,0) {
            \includegraphics[width=\linewidth]{figures/tangent/hyp_manifold_means.pdf}
        };
        % \node[anchor=north west, fill=white, fill opacity=0.7, text opacity=1, inner sep=2pt] at (image.north west) {\textbf{(b)}};
    \end{tikzpicture}
\end{minipage}%
% Subfigure (c): Hyperbolic Means
\begin{minipage}[t]{0.33\linewidth}
    \centering
    \begin{tikzpicture}
        \node[anchor=south west, inner sep=0] (image) at (0,0) {
            \vspace{-2ex}
            \includegraphics[width=\linewidth]{figures/tangent/hyp_projection2d_obj.pdf}
        };
        % \node[anchor=north west, fill=white, fill opacity=0.7, text opacity=1, inner sep=2pt] at (image.north west) {\textbf{(e)}};
    \end{tikzpicture}
\end{minipage}

\vspace{-1ex} % Adds a clean vertical gap between the two rows

% ==================================================================
% ROW 2: TANGENT PROJECTIONS (WITH ARROWS)
% ==================================================================
% Subfigure (d): Euclidean Tangent
\begin{minipage}[t]{0.33\linewidth}
    \centering
    \begin{tikzpicture}
        \node[anchor=south west, inner sep=0] (image) at (0,0) {
            \vspace{-2ex}
            \includegraphics[width=\linewidth]{figures/tangent/sph_tangent_attribute_directions.pdf}
        };
        \node[anchor=south, fill=white, fill opacity=0.7, text opacity=1, inner sep=2pt] at (image.south) {
            Spherical
        };
    \end{tikzpicture}
\end{minipage}%
% Subfigure (e): Spherical Tangent
\begin{minipage}[t]{0.33\linewidth}
    \centering
    \begin{tikzpicture}
        \node[anchor=south west, inner sep=0] (image) at (0,0) {
            \includegraphics[width=\linewidth]{figures/tangent/hyp_tangent_attribute_directions.pdf}
        };
        % \node[anchor=north west, fill=white, fill opacity=0.7, text opacity=1, inner sep=2pt] at (image.north west) {\textbf{(d)}};
        \node[anchor=south, fill=white, fill opacity=0.7, text opacity=1, inner sep=2pt] at (image.south) {
            Hyperbolic
        };
    \end{tikzpicture}
\end{minipage}%
% Subfigure (f): Hyperbolic Tangent
\begin{minipage}[t]{0.33\linewidth}
    \centering
    \begin{tikzpicture}
        \node[anchor=south west, inner sep=0] (image) at (0, 0) {
            \includegraphics[width=\linewidth]{figures/tangent/hyp_projection2d_attr.pdf}
        };
        % \node[anchor=north west, fill=white, fill opacity=0.7, text opacity=1, inner sep=2pt] at (image.north west) {\textbf{(f)}};
        \node[anchor=south, fill=white, fill opacity=0.7, text opacity=1, inner sep=2pt] at (image.south) {
            Poincar\'e Projection
        };
    \end{tikzpicture}
\end{minipage}


==> figures/taxanomy/with_euc.tex <==
% Model taxonomy figure (with Euclidean column, Euclidean leftmost)
% Requires: tikz, tikzlibrary{positioning,fit,backgrounds,decorations.pathreplacing}
\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
  font=\sffamily,
  geombox/.style={
    rounded corners=6pt,
    draw,
    line width=1.6pt,
    minimum height=2.0em,
    text depth=0.3ex,
    inner xsep=10pt,
    align=center,
    font=\sffamily\bfseries\large,
  },
  modelcard/.style 2 args={
    rounded corners=5pt,
    draw=#1,
    fill=#1!12,
    line width=2pt,
    minimum width=3.8cm,
    minimum height=3.6cm,
    align=center,
    font=\sffamily,
    text=#2,
  },
  anno/.style={->, >=stealth, thick, gray},
  brace/.style={decorate, decoration={brace, amplitude=6pt}, thick, gray},
]

%% ── Column x-positions ──────────────────────────────────────────
\def\xDINOE{0}      % Euclidean DINOv2-raw (leftmost)
\def\xCLIP{5.6}
\def\xCLIPB{10.0}
\def\xMERU{15.6}
\def\xHyCo{20.0}

%% ── Model cards ─────────────────────────────────────────────────

% DINOv2 raw (Euclidean)
\node[modelcard={teal!70!black}{teal!60!black}] (DINOE) at (\xDINOE,0) {
  {\bfseries\large DINOv2}\\[4pt]
  \textit{\small LVD-142M}\\[2pt]
  Vision-Only
};
% \node[below=0.15cm of DINOE, font=\sffamily\small\itshape, text=teal!70!black]
  (dinoEraw) {(unnormalized)};

% CLIP ViT-L
\node[modelcard={blue!70!cyan}{blue!80!black}] (CLIP) at (\xCLIP,0) {
  {\bfseries\large OpenAI-CLIP}\\[4pt]
  400M pairs\\[2pt]
  \textit{\small Contrastive}
};

% CLIP-B
\node[modelcard={green!60!black}{green!40!black}] (CLIPB) at (\xCLIPB,0) {
  {\bfseries\large CLIP}\\[4pt]
  20.5M (GRIT)\\[2pt]
  \textit{\small Contrastive}
};

% MERU
\node[modelcard={orange!80!red}{orange!60!black}] (MERU) at (\xMERU,0) {
  {\bfseries\large MERU}\\[4pt]
  20.5M (GRIT)\\[2pt]
  \textit{\small Language-Vision} \\[2pt]
  \textit{\small Entailment}
};

% HyCoCLIP
\node[modelcard={red!70!orange}{red!60!black}] (HyCo) at (\xHyCo,0) {
  {\bfseries\large HyCoCLIP}\\[4pt]
  20.5M (GRIT)\\[2pt]
  \textit{\small Scene-Object} \\[2pt]
  \textit{\small Language-Vision} \\[2pt]
  \textit{\small Entailment}
};

%% ── Geometry header boxes ────────────────────────────────────────

% Euclidean header (DINOv2 raw only)
\node[geombox,
      draw=teal!60!black,
      fill=teal!6,
      text=teal!70!black,
      fit={($(DINOE.north west)+(-0.18,0.55)$)($(DINOE.north east)+(0.18,0.55)$)},
      minimum height=1.75em,
      ] (eucHeader) {\raisebox{-1ex}{Euclidean $\bigl(\mathbb{R}^{d}\bigr)$}};

% Spherical header (spans CLIP, CLIP-B)
\node[geombox,
      draw=blue!50!cyan,
      fill=blue!6,
      text=blue!70!cyan,
      fit={($(CLIP.north west)+(-0.18,0.55)$)($(CLIPB.north east)+(0.18,0.55)$)},
      minimum height=1.75em,
      ] (sphereHeader) {\raisebox{-1ex}{Spherical $\bigl(\mathbb{S}^{d-1}\bigr)$}};

% Hyperbolic header (spans MERU, HyCoCLIP)
\node[geombox,
      draw=green!55!black,
      fill=green!6,
      text=green!50!black,
      fit={($(MERU.north west)+(-0.18,0.55)$)($(HyCo.north east)+(0.18,0.55)$)},
      minimum height=1.75em,
      ] (hypHeader) {\raisebox{-1ex}{Hyperbolic $\bigl(\mathbb{H}^d_\kappa\bigr)$}};

%% ── Annotations below cards ──────────────────────────────────────
% \node[below=0.625cm of CLIP, font=\sffamily\small, text=gray, align=center]
%   (annoCLIP) {Vision-Language};
% \draw[anno] (annoCLIP.north) -- (CLIP.south);

% \node[below=0.65cm of DINOE, font=\sffamily\small, text=gray, align=center]
%   (annoDINOE) {Vision Only};
% \draw[anno] (annoDINOE.north) -- (dinoEraw.south);

%% ── GRIT bracket ─────────────────────────────────────────────────
\coordinate (brL) at ($(CLIPB.south west)+(0,-0.4)$);
\coordinate (brR) at ($(HyCo.south east)+(0,-0.4)$);
\draw[brace] (brR) -- (brL)
  node[midway, below=8pt, font=\sffamily\small\bfseries, text=gray, align=center]
  {Same ViT backbone + GRIT data $\rightarrow$ isolates geometry effect};

\end{tikzpicture}%
}
\vspace{-4ex}
\caption{%
  \textbf{Model taxonomy.}
  Five model configurations span three embedding geometries.
  DINOv2 is included with raw, unnormalised features (Euclidean $\mathbb{R}^d$).
  The CLIP / MERU / HyCoCLIP triple shares the same ViT-B backbone and GRIT
  pretraining data, isolating embedding geometry as the sole varying factor.%
}
\label{fig:taxonomy_euclidean}
\end{figure}


==> figures/taxanomy/without_euc.tex <==
% Model taxonomy figure (no Euclidean column)
% Requires: tikz, tikzlibrary{positioning,fit,backgrounds}
\begin{figure}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
  font=\sffamily,
  % Geometry header boxes
  geombox/.style={
    rounded corners=6pt,
    draw,
    line width=1.6pt,
    minimum height=2.0em,
    text depth=0.3ex,
    inner xsep=10pt,
    align=center,
    font=\sffamily\bfseries\large,
  },
  % Model card style
  modelcard/.style 2 args={
    rounded corners=5pt,
    draw=#1,
    fill=#1!12,
    line width=2pt,
    minimum width=3.8cm,
    minimum height=3.6cm,
    align=center,
    font=\sffamily,
    text=#2,
  },
  % Annotation arrow
  anno/.style={->, >=stealth, thick, gray},
  % Bracket
  brace/.style={decorate, decoration={brace, amplitude=6pt}, thick, gray},
]

%% ── Column x-positions ──────────────────────────────────────────
\def\xCLIP{0}
\def\xDINO{4.4}
\def\xCLIPB{8.8}
\def\xMERU{14.4}
\def\xHyCo{19.0}

%% ── Model cards ─────────────────────────────────────────────────
% CLIP ViT-L
\node[modelcard={blue!70!cyan}{blue!80!black}] (CLIP) at (\xCLIP,0) {
  {\bfseries\large CLIP}\\[4pt]
  ViT-L/14\\
  400M pairs\\[2pt]
  \textit{\small Contrastive}
};

% DINOv2 ViT-L
\node[modelcard={violet}{violet!80!black}] (DINO) at (\xDINO,0) {
  {\bfseries\large DINOv2}\\[4pt]
  ViT-L/14\\
  LVD-142M\\[2pt]
  \textit{\small Self-distillation}
};
% DINOv2-raw sub-label
\node[below=0.15cm of DINO, font=\sffamily\small\itshape, text=violet!70!black]
  (dinoraw) {(normalized)};

% CLIP-B
\node[modelcard={green!60!black}{green!40!black}] (CLIPB) at (\xCLIPB,0) {
  {\bfseries\large CLIP-B}\\[4pt]
  ViT-B/16\\
  20.5M (GRIT)\\[2pt]
  \textit{\small Contrastive}
};

% MERU
\node[modelcard={orange!80!red}{orange!60!black}] (MERU) at (\xMERU,0) {
  {\bfseries\large MERU}\\[4pt]
  ViT-B/16\\
  20.5M (GRIT)\\[2pt]
  \textit{\small Hyperbolic}\\
  \textit{\small Contrastive}
};

% HyCoCLIP
\node[modelcard={red!70!orange}{red!60!black}] (HyCo) at (\xHyCo,0) {
  {\bfseries\large HyCoCLIP}\\[4pt]
  ViT-B/16\\
  20.5M (GRIT)\\[2pt]
  \textit{\small Hyperbolic}\\
  \textit{\small Contrastive Supervised}
  };

%% ── Geometry header boxes ────────────────────────────────────────
% Spherical header (spans CLIP, DINO, CLIP-B)
\node[geombox,
      draw=blue!50!cyan,
      fill=blue!6,
      text=blue!70!cyan,
      fit={($(CLIP.north west)+(-0.18,0.55)$)($(CLIPB.north east)+(0.18,0.55)$)},
      minimum height=1.75em,
] (sphereHeader) {\raisebox{-1ex}{Spherical $\bigl(\mathbb{S}^{d-1}\bigr)$}};

% Hyperbolic header (spans MERU, HyCoCLIP)
\node[geombox,
      draw=green!55!black,
      fill=green!6,
      text=green!50!black,
      fit={($(MERU.north west)+(-0.18,0.55)$)($(HyCo.north east)+(0.18,0.55)$)},
      minimum height=1.75em,
      ] (hypHeader) {\raisebox{-1ex}{Hyperbolic $\bigl(\mathbb{H}^d_\kappa\bigr)$}};

%% ── Annotations below cards ──────────────────────────────────────
\node[below=0.625cm of CLIP, font=\sffamily\small, text=gray, align=center]
  (annoCLIP) {Vision-Language};

\node[below=0.65cm of DINO, font=\sffamily\small, text=gray, align=center]
  (annoDINO) {Vision Only};
% \draw[anno] (annoDINO.north) -- (dinoraw.south);

%% ── GRIT bracket ─────────────────────────────────────────────────
\coordinate (brL) at ($(CLIPB.south west)+(0,-0.4)$);
\coordinate (brR) at ($(HyCo.south east)+(0,-0.4)$);
\draw[brace] (brR) -- (brL)
  node[midway, below=8pt, font=\sffamily\small\bfseries, text=gray, align=center]
  {Same ViT-B backbone + GRIT data\\$\rightarrow$ isolates geometry effect};

% %% ── Research question ────────────────────────────────────────────
% \node[below=1.75cm of $(MERU.south)!0.5!(HyCo.south)$,
%       font=\sffamily\itshape, text=gray!80!black]
%   {Does geometry matter? \textit{(Spherical vs.\ Hyperbolic)}};

\end{tikzpicture}%
}
\caption{%
  \textbf{Model taxonomy.}
  The five models evaluated span two embedding geometries (spherical, hyperbolic) and
  two supervision regimes (vision-language and vision-only).
  DINOv2 is evaluated both with standard $\ell_2$ normalisation to project to the spherical geometry.
  The CLIP-B / MERU-B / HyCoCLIP-B triple shares the same ViT-B backbone and GRIT
  pretraining data, isolating embedding geometry as the sole varying factor.%
}
\label{fig:taxonomy}
\end{figure}


==> sections/2_preliminary_tat.tex <==
\newpage

\setlength{\belowdisplayskip}{5pt} \setlength{\belowdisplayshortskip}{5pt}
\setlength{\abovedisplayskip}{5pt} \setlength{\abovedisplayshortskip}{5pt}

\section{Preliminaries}%\label{sec:prelim}
\begin{comment}
In this section, we provide a brief overview of %the GDE framework and 
the mathematical background relevant to the notion of compositional embeddings.
\end{comment}
In this section, we provide a brief overview of the mathematical background relevant to the notion of compositional embeddings and the GDE framework.

Large-scale multi-modal models encode images $x \in \mathcal{X}$ and their associated descriptive text $y\in\mathcal{Y}$ into shared embedding spaces via specific encoders $\phi_{im}:\mathcal{X} \rightarrow \mathbb{R}^d$, $\phi_{tx}:\mathcal{Y} \rightarrow \mathbb{R}^d$. We indicate with $\mathcal{M}\subset\mathbb{R}^d$ the target $d$-dimensional representation manifold, and with $\mathbf{u}\in\mathcal{M}$ a generic point on the manifold. Given $N$ samples, their intrinsic (Fr\'echet) mean is 
$\boldsymbol{\mu} =
    \arg\min_{\mathbf{u}\in\mathcal{M}}
    \sum_{i=1,\ldots N}
    d_{\mathcal{M}}(\mathbf{u},\mathbf{u}_i)^2$,
%\end{equation}
where $d_{\mathcal{M}}$ denotes the geodesic distance on the manifold. Let $T_{\boldsymbol{\mu}}\mathcal{M}$ be the tangent space to the embedding manifold in $\boldsymbol{\mu}$, and $\mathbf{t}_i = \mathrm{Log}_{\boldsymbol{\mu}}(\mathbf{u}_i) \in T_{\boldsymbol{\mu}}\mathcal{M}$ the projection of an embedding vector to the tangent space via the \emph{logarithmic map}. The function is locally invertible, and its inverse is the \emph{exponential map}  $\mathbf{u}_i = \mathrm{Exp}_{\boldsymbol{\mu}}(\mathbf{t}_i) \in \mathcal{M}$.  
%that sends straight lines of the tangent plane into geodesic curves of the manifold. 

The exact form of the map functions depends on the manifold's geometry %.
and prior work has focused on contrastive language-image models as CLIP, based on spherical representation embeddings. In this case, the standard inner product is $s_{\mathrm{sph}}(\mathbf{u},\mathbf{u'}) = \langle\mathbf{u}, \mathbf{u'}\rangle = \mathbf{u}^\top \mathbf{u'}$, while the mappings are 
\begin{align}
  \mathrm{Log}_{\boldsymbol{\mu}}(\mathbf{u})
    &=
    \arccos(\boldsymbol{\mu}^\top\mathbf{u})
    \frac{
      \mathbf{u} - (\boldsymbol{\mu}^\top\mathbf{u})\boldsymbol{\mu}
    }{
      \|\mathbf{u} - (\boldsymbol{\mu}^\top\mathbf{u})\boldsymbol{\mu}\|
    },
  &
  \mathrm{Exp}_{\boldsymbol{\mu}}(\mathbf{t})
    &=
    \cos(\|\mathbf{t}\|)\boldsymbol{\mu}
    +
    \sin(\|\mathbf{t}\|)
    \frac{\mathbf{t}}{\|\mathbf{t}\|}~.
  \label{eq:sphere_maps}
\end{align}

\tat{go ahead here to explain GDE-pairs and text-based solutions}


For Euclidean manifolds, the tangent space at every point is naturally identified with the manifold itself. In this case, the logarithmic and exponential maps reduce to ordinary subtraction and addition:  
$\mathrm{Log}_{\boldsymbol{\mu}}(\mathbf{u}) = \mathbf{u}-\boldsymbol{\mu}$, 
$\mathrm{Exp}_{\boldsymbol{\mu}}(\mathbf{t})= \boldsymbol{\mu}+\mathbf{t}$.
The sample similarity on the manifold is simply expressed by the cosine similarity 
$s_{\mathrm{euc}}(\mathbf{u},\mathbf{u'}) = \mathbf{u}^\top\mathbf{u'}/\|\mathbf{u}\|\,\|\mathbf{u'}\|$.

\begin{comment}
\begin{align}
  \mathrm{Log}_{\boldsymbol{\mu}}(\mathbf{u})
    &=
    \mathbf{u}-\boldsymbol{\mu},
  &
  \mathrm{Exp}_{\boldsymbol{\mu}}(\mathbf{t})
    &=
    \boldsymbol{\mu}+\mathbf{t},
  &
  s_{\mathrm{euc}}(\mathbf{u},\mathbf{u'})
    =
    \frac{
        \mathbf{u}^\top\mathbf{u'}
    }{
        \|\mathbf{u}\|\,\|\mathbf{u'}\|
    }~.
  \label{eq:euc_maps}
\end{align}
\end{comment}

For spherical embeddings, the %mappings are
similarity function is the standard inner product $s_{\mathrm{sph}}(\mathbf{u},\mathbf{u'}) = \langle\mathbf{u}, \mathbf{u'}\rangle = \mathbf{u}^\top \mathbf{u'}$, while the mappings are 
\begin{align}
  \mathrm{Log}_{\boldsymbol{\mu}}(\mathbf{u})
    &=
    \arccos(\boldsymbol{\mu}^\top\mathbf{u})
    \frac{
      \mathbf{u} - (\boldsymbol{\mu}^\top\mathbf{u})\boldsymbol{\mu}
    }{
      \|\mathbf{u} - (\boldsymbol{\mu}^\top\mathbf{u})\boldsymbol{\mu}\|
    },
  &
  \mathrm{Exp}_{\boldsymbol{\mu}}(\mathbf{t})
    &=
    \cos(\|\mathbf{t}\|)\boldsymbol{\mu}
    +
    \sin(\|\mathbf{t}\|)
    \frac{\mathbf{t}}{\|\mathbf{t}\|}~.
  \label{eq:sphere_maps}
\end{align}
%The corresponding similarity function is the standard inner product $s_{\mathrm{sph}}(\mathbf{u},\mathbf{u'}) = \mathbf{u}^\top \mathbf{u'}$.

Hyperbolic models embed representations on the Lorentz space, where the Lorentzian inner product is
$\langle\mathbf{u},\mathbf{u'}\rangle_{\mathcal{L}}
=
\sum_{i=1}^{d}u_iu'_i -u_0u'_0$ and corresponds to the sample similarity function $s_{\mathrm{hyp}}(\mathbf{u},\mathbf{u'})$.
The logarithmic and exponential maps are defined as:
\begin{gather}
  \mathrm{Log}_{\boldsymbol{\mu}}(\mathbf{u})
    =
    \frac{
      \mathrm{arccosh}\big(
      -\langle\boldsymbol{\mu},\mathbf{u}\rangle_{\mathcal{L}}
      \big)
    }{
      \sqrt{
      \langle\boldsymbol{\mu},\mathbf{u}\rangle_{\mathcal{L}}^2 - 1
      }
    }
    \Big(
      \mathbf{u}
      +
      \langle\boldsymbol{\mu},\mathbf{u}\rangle_{\mathcal{L}}\boldsymbol{\mu}
    \Big),
  \\
  \mathrm{Exp}_{\boldsymbol{\mu}}(\mathbf{t})
    =
    \cosh(\|\mathbf{t}\|_{\mathcal{L}})\boldsymbol{\mu}
    +
    \sinh(\|\mathbf{t}\|_{\mathcal{L}})
    \frac{\mathbf{t}}{\|\mathbf{t}\|_{\mathcal{L}}}, \quad \text{where} \quad \|\mathbf{t}\|_{\mathcal{L}}
=
\sqrt{\langle\mathbf{t},\mathbf{t}\rangle_{\mathcal{L}}}~.
\end{gather} 

\section{Geodesically Decomposable Embeddings} 
Given an image dataset with attribute-object annotations $\mathcal{D}=\{x_i,a_i,o_i\}_{i=1}^N$ where $a_i\in\mathcal{A}$ and $o_i\in\mathcal{O}$ are respectively the attribute and object labels and $\boldsymbol{\mu}$ defines their intrinsic mean, GDE calculates independent primitive semantic directions in the tangent space $T_{\boldsymbol{\mu}}\mathcal{M}$. They are obtained as a weighted average of the tangent projected vectors that originate from the images sharing a certain attribute or vector:
\begin{align}
    \mathbf{v}_a
    &=
    \frac{
        \sum_{i\in S_a}
        w_i\mathbf{t}_i
    }{
        \sum_{i\in S_a}
        w_i
    },
    \qquad
    S_a
    =
    \{i : a_i=a\},
    &
    \mathbf{v}_o
    &=
    \frac{
        \sum_{i\in S_o}
        w_i\mathbf{t}_i
    }{
        \sum_{i\in S_o}
        w_i
    },
    \qquad
    S_o
    =
    \{i : o_i=o\}~.
    %\label{eq:gde_weighted}
\end{align}
Following~\cite{berasiNotOnlyText2025a}, the weights 
\tat{
$w_i
    \propto
    \exp\!\,(
            \phi_{im}(x_i)^\top
            {\phi_{tx}}(a_i,o_i)/\tau
    )$}
rescale each term according to
its alignment with the corresponding attribute-object text representation $\phi_{tx}(a_i,o_i)$ via cosine similarity and the temperature parameter $\tau$.

To infer the label of a test sample $x$ with embedding $\mathbf{u}_x$, we can exploit the \emph{GDE primitives} by projecting the sample to the tangent space via the logarithmic map to obtain $\mathbf{t}_x$ and then searching for the most similar primitive directions 
\begin{equation}
\hat{a}=\arg\max_{a\in\mathcal{A}}\frac{\mathbf{v}_a^\top \mathbf{t}_x}{\|\mathbf{v}_a\|\|\mathbf{t}_x\|}\, , \quad \hat{o}=\arg\max_{o\in\mathcal{O}}\frac{\mathbf{v}_o^\top \mathbf{t}_x}{\|\mathbf{v}_o\|\|\mathbf{t}_x\|}~.
\end{equation}
Alternatively, we can use the \emph{GDE pairs} strategy, by considering the addition vector in the tangent space $\textbf{v}_{(a,o)}=\textbf{v}_{a}+\textbf{v}_{o}$ which is projected back to the original manifold $\tilde{\textbf{u}}_{(a,o)}=\mathrm{Exp}_\mu(\textbf{v}_{(a,o)})$ where it is used as reference for the test sample, searching for the nearest object-attribute prototype:
\begin{equation}
(\hat{a}, \hat{o})=\arg\max_{a,o \in \{\mathcal{A}\times\mathcal{O}\}}\langle\mathbf{u}_x,\tilde{\textbf{u}}_{(a,o)}\rangle~.
\end{equation}

\tat{It might be better to present the GDE pairs first and then the GDE primitives}

\medskip
\tat{there is something I'm not sure about. The prediction for the GDE primitives is based on a comparison in the tangent space. The prediction for the GDE pairs happens instead in the original manifold space. Did I understand correctly?
}

\medskip
\tat{Note that I would not explicitly describe how to calculate the score for the group robustness case. As we want to pass the message that it is an application we will mention that score directly in the experimental section, explaining that is simply a variant of the formulas that appear here.}

\section{Intrinsic Primitives}

\section{Zero-Shot, text-based solution} 
